Teaching Erlang through the Internet: An Experience Report

Today functional programming languages are seen as a practical solution to the difficult problems of concurrent and distributed programming. Erlang is a functional language designed to build massively scalable and fault tolerant applications. This paper describes the authors' experiences delivering a massively online open course (MOOC) on the FutureLearn platform.

==> eptcsdata.tex <==
\providecommand{\firstpage}{52}
\providecommand{\publicationstatus}{S. Thompson (Ed.): TFPIE 2017.\\
EPTCS 270, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.270.4}{10.4204/EPTCS.270.4}}
\pdfoutput=1

